Maximizing performance with an eye on the finances: a chance-constrained model for football transfer market decisions

Composing a team of professional players is among the most crucial decisions in association football. Nevertheless, transfer market decisions are often based on myopic objectives and are questionable from a financial point of view. This paper introduces a chance-constrained model to provide analytic support to club managers during transfer windows. The model seeks a top-performing team while adapting to different budgets and financial-risk profiles. In addition, it provides a new rating system that is able to numerically reflect the on-field performance of football players and thus contribute to an objective assessment of football players. The model and rating system are tested on a case study based on real market data. The data from the case study are available online for the benefit of future research.

==> tablesChelsea.tex <==
 \begin{longtable}{ccccccccc}
    \label{tab:cs:realB}\\
  \caption{Players bought by Chelsea FC in real-life and suggested by the model with different values of $\alpha$ and $R$. $B$ indicates that the player is bought. Values are in million Euro.}\\
    \toprule
    \multirow{ 2}{*}{Player} & \multirow{ 2}{*}{Value} & \multirow{ 2}{*}{Rating} & \multirow{ 2}{*}{Age}&\multirow{ 2}{*}{Actual} &\multicolumn{4}{c}{$\alpha$-$R$}\\
     &  &  & & & $0.2-1$& $0.2-1.2$ & $0.8-1$&$0.8-1.2$\\
    \midrule
    Diego Costa & 31.50 &0.126064&25 & B&&& &\\
    Cesc F\`{a}bregas & 45.00 & 0.288742&27& B&B&B&B&\\
    Filipe Lu\'{i}s & 13.50 &0.160814&28 & B&B&&B &\\
    Lo\"{i}c R\'{e}my & 10.80 &0.109193 &27& B&&B& &B \\
    Mario Pasalic &2.70 & -0.056862&19& B &&& &B\\
    Didier Drogba & 2.03 &0.078912 &36& B&&&B &B\\
    Alexis S\'{a}nchez & 27.00 &0.233056 &25& &B&B&B &B\\
    Danny Welbeck & 15.30 & 0.155037&23& & B&B&B &B\\
    David Ospina &4.5&0.086959 &25& &B&B&B & B\\
    Fernando & 15.75& 0.160701&26& &B&B&B &B\\
    Bacary Sagna & 10.80& 0.129089&31& &B&B& &\\
    Ander Herrera &18.00& 0.150451&24& &B&& &\\
    Daley Blind & 10.80& 0.173537&24& &B&B&B & B \\
    \'{A}ngel Di Mar\'{i}a & 45.00&0.261691 &26& &B&& &\\
    Mathieu Debuchy &9.0 &0.123112&28& & & & B &\\
    Calum Chambers & 1.80 & 0.008474 &19& & & & & B\\
    Eliaquim Mangala & 25.20&0.093491 &23& & & & & B\\
    Bruno Zuculini & 3.60 & 0.003938  &21& & & & & B\\
    Marcos Rojo & 10.80& 0.082198 &24& & & & & B\\
    Siem de Jong & 9.00& 0.166799 &25& & & & & B \\
    \bottomrule
  \end{longtable}

\begin{longtable}{ccccccccc}
    \label{tab:cs:realS}\\
  \caption{Players sold for the case of Chelsea FC in real-life and suggested by the model with different values of $\alpha$ and $R$. $B$ indicates that the player is bought. Values are in million Euro.}\\
    \toprule
    \multirow{ 2}{*}{Player} & \multirow{ 2}{*}{Value} & \multirow{ 2}{*}{Rating} & \multirow{ 2}{*}{Age}&\multirow{ 2}{*}{Actual} &\multicolumn{4}{c}{$\alpha$-$R$}\\
     &  &  & & & $0.2-1$& $0.2-1.2$ & $0.8-1$&$0.8-1.2$\\
    \midrule
David Luiz  &23.400 & 0.186949 & 27&S& & & & \\
Romelu Lukaku & 22.500&0.133427 &21 &    S& & & & \\
Demba Ba   &9.900& 0.120763 &  28 & S& & & S& \\
Patrick van Aanholt&   3.150& 0.0503757&  23  &S& S& & & \\
Frank Lampard   &1.800 & 0.141603 & 35 & S & & & S& \\
Ashley Cole   &4.500  & 0.134776 &32 & S & S& &  S&S\\
Samuel Eto'o   &8.100 & 0.144796& 32  & S & & & &S\\
Henrique Hil\`{a}rio& 0.225& -0.070385& 38  &  S &S & S& S& \\
Jhon P\'{i}rez & NA & NA& 21&S & & & & \\
Milan Lalkovic & 0.225 &NA &21&S & & & & \\
Sam Hutchinson & 0.135 & NA&24&S & & & & \\
Petr Cech & 25.00 & 0.196171 &31 && & & & S\\
John Terry & 12.00 & 0.167619 &31& & & & & S\\
Branislav Ivanovic & 24.00 & 0.220976& 29& & & & & S\\
Michael Essien & 10.00 & 0.172794 &30& & & & & S\\
Fernando Torres & 28.00 & 0.136716 &29& & &S & & S\\
Mark Schwarzer & 1.00 & 0.040236 &40& &S & S& S& \\
Kurt Zouma & 7.00 & 0.029078 &18& & & & S& \\
Juan Mata& 42.00 & 0.190657 &25& & S& S& S& \\
Oscar & 32.00 & 0.169947 & 21 & &S & & S& \\
Eden Hazard & 40.00 & 0.204971 &22& &S & S& S& \\
Andr\'{e} Sch\"{u}rrle& 25.00 & 0.191104 &22& & S& & S& \\
Ryan Bertrand & 5.00 &  0.076529&23& &S &S & & \\
Ramires & 27.00 & 0.144788 &26& &S &S & & \\
Willian & 35.00 & 0.198471 &24& & S&S & & \\
Tom\'{a}s Kalas& 6.00 & 0.039281 &20& & S& & & \\
Nemanja Matic& 14.00 &  0.136384&24& &S & & & \\
Kevin De Bruyne& 10.00 & 0.066263 &22& &S & & & \\
Marko Marin& 7.00 &0.052772 &24& &S & & & \\
Ulises D\'{a}vila& 1.50 & 0.011584 &22& &S & & & \\
Lucas-Piaz\'{o}n& 5.00 & 0.051867 &19& &S & & & \\
Victor Moses& 15.00 & 0.094867 &22& &S & & & \\
Mohamed Salah& 6.50 & 0.064382 &21& &S & & & \\
 \bottomrule
  \end{longtable}
  
